Symbolic Runtime Verification for Monitoring under Uncertainties and Assumptions

Runtime Verification deals with the question of whether a run of a system adheres to its specification. This paper studies runtime verification in the presence of partial knowledge about the observed run, particularly where input values may not be precise or may not be observed at all. We also allow declaring assumptions on the execution which permits to obtain more precise verdicts also under imprecise inputs. To this end, we show how to understand a given correctness property as a symbolic formula and explain that monitoring boils down to solving this formula iteratively, whenever more and more observations of the run are given. We base our framework on stream runtime verification, which allows to express temporal correctness properties not only in the Boolean but also in richer logical theories. While in general our approach requires to consider larger and larger sets of formulas, we identify domains (including Booleans and Linear Algebra) for which pruning strategies exist, which allows to monitor with constant memory (i.e. independent of the length of the observation) while preserving the same inference power as the monitor that remembers all observations. We empirically exhibit the power of our technique using a prototype implementation under two important cases studies: software for testing car emissions and heart-rate monitoring.

==> implementation.tex <==
 \section{Implementation}
 
%  \begin{itemize}
%   \item Algorithmic description of approach
%  \end{itemize}


==> uncertCalc.tex <==
\section{Monitoring Uncertainty}

%\input{cesar}
% \begin{itemize}
%  \item Idea of symbolic calculation (high level)
%  \item Idea of rewriting formuals
%  \item Picture visualizing calculation of monitor
%  \item Formal framework for “Basis changes”
%  \begin{itemize}
%   \item boolean case
%   \item real case with proofs refering to Soundness/Completeness
%   \item restrictions/combinition of real/bool -> not complete with finite memory
%   \item other theories
%  \end{itemize}
%  \item Proof of perfectness under certain conditions
%  \item Extensions which may cause imperfectness, and how they are handled (if, variable ranges 	(example of shape which cannot be expressed by two vectors)
% \end{itemize}


In this section we intruduce a technique to monitoring using symbolic
computation.
%
We first show that existing monitoring approaches for monitoring with
all input values known (certainty) for past only specifications are an
instance of our framework that uses substitution and evaluation.
%
This fragment of monitoring languages is called the very efficient
monitoring fragment.
%
Similarly, monitoring approaches that allow bounded future references
are also an instance of the framework were resolving equations may
require to wait for all the input values to be present (this fragment
is called efficient monitoring).
%
In both cases, all previous work assumes that input values are known
and do not allow to anticipate and to improve the monitoring using
assumptions.

In order to handle uncertainties our monitors store equations that
include variables that capture the unknown information, for example
the unknown input values.
%
Therefore, the memory that the monitors need can grow without bound if
number of uncertain items also grows without bound.
%
Therefore, \emph{perfect monitoring under uncertainty is not trace
  length independent even for past only specifications for rich data
  domains.}
%
In this section we also instantiate the framework to concrete
theories, namely Booleans and LA (linear arithmatic) and show the
theories and conditions under which how to construct bounded perfect
monitors under unbounded imperfect information.
%
Finally, we will show that anticipation can be obtained by
instantiating the equations of the desired output ahead of time.
%
If the result is inevitable (for the observed input and the
constraints) the monitor will infer the inevitable outcome ahead of
time.

\subsection{Basic symbolic approach to handle uncertainty}

As previously mentioned a drawback of calculating with the common abstract domains $\mathbb{B}^\#$ and $\mathbb{R}^\#$ is that the origin of the abstracted values gets lost (see \autoref{fig:lolaIntroEx2}).
A straight-forward approach to overcome this issue is to use symbolic formulas over the unknown input events to express the potential stream values, preserving the interconnection, as shown in \autoref{fig:lolaIntroEx3}.

In this paper we apply the approach of symbolic calculation on stream transformations and show how an uncertain stream transformation function can be generated from a LOLA specification and how a monitor can be genrated. Our approach is based on the idea that every stream event successively gets a symbolic value assigned which can be evaluated under a set of global constraints.

First we give a formal definition of the symbolic formulas we use as event values:

\begin{definition}[Symbolic formulas]
$\mathbb{D}^\star$ denotes symbolic formulas over atomic propositions $\mathcal{A}$ with given types and can be recursively defined as\\

$\mathbb{D}^\star = c \mid a \mid f(\mathbb{D}_1^\star, ..., \mathbb{D}_n^\star) \mid ite(\mathbb{B}^\star, \mathbb{D}^\star, \mathbb{D}^\star)$\\
 
for $c$ a constant of type $\mathbb{D}$, $a \in \mathcal{A}$ an atomic proposition of type $\mathbb{D}$, $f$ a total function $\mathbb{D}_1 \times \dots \times \mathbb{D}_n \rightarrow \mathbb{D}$.
\end{definition}

We call a set of constraints from $\mathbb{B}^\star$ a \textit{Boolean constraint set}. Note that constraints from a Boolean constraint set may also reference variables of type real, e.g. $x \geq 5$.\\
For a formula $\varphi \in \mathbb{D}^\star$ we write $\llbracket \varphi \rrbracket_\mathcal{C}$ to denote the set of values $\varphi$ evaluates to for variable assignments that satisfy all constraints in $\mathcal{C}$, i.e. $\llbracket \varphi \rrbracket_\mathcal{C} = \{v | \exists s: s \models \mathcal{C} \cup \{ \varphi = v \} \}$

Note that in general a set of (even finite) input streams $S \in 2^{\mathcal{S}_{\mathbb{D}_1} \times \dots \times \mathcal{S}_{\mathbb{D}_n}}$ may not be describable by finitely many constraints. Since such sets are of little practical relevance, as they cannot be handled with finite memory we restrict in the following work on uncertain input streams, where every prefix of the stream can be expressed by a finite set of boolean constraints:

\begin{definition}[Finitely describable stream set]
 A set of tuples of concrete streams $\Sigma \in 2^{\mathcal{S}_{\mathbb{D}_1} \times \dots \times \mathcal{S}_{\mathbb{D}_n}}$ is called \textit{finitely describable},
 if there is a Stream $\sigma \in \mathcal{S}_{\mathbb{B}^\star}$ of boolean constraint sets over finite subsets of $\mathcal{A} = \{s^t | s \in \mathcal{S}_i, t \in \mathbb{T}\}$, such that
 
 \begin{itemize}
  \item $\forall (s_1, \dots, s_n) \in \Sigma: \forall t \in \mathbb{T}: (\forall i \leq t: s_1^i = s_1(i) \land ... \land s_n^i = s_n(i)) \models \sigma(t)$
  \item $\forall t \in \mathbb{T}: \sigma(t) \subseteq \sigma(t + 1)$\todo{Better model as stream which only contains the difference}
 \end{itemize}

\end{definition}

For the example from \cref{fig:lolaIntroEx3} one would receive the following finite stream description:\\

\noindent
$\langle \{1 \leq x^0 \land x^0 \leq 5\}, 
         \{1 \leq x^0 \land x^0 \leq 5, x^1 = 4\}, 
         \{1 \leq x^0 \land x^0 \leq 5, x^1 = 4,\\ x^2 = 5\}, 
         \{1 \leq x^0 \land x^0 \leq 5, x^1 = 4, x^2 = 5, x^3 = 7\} \dots \rangle$\\

Due to the subset relation of the elements it is sufficent to denote only the difference of each constraint set to the last one:\\

\noindent
$\langle \{1 \leq x^0 \land x^0 \leq 5\}, 
         \{x^1 = 4\}, 
         \{x^2 = 5\}, 
         \{x^3 = 7\} \dots \rangle$\\

Based on the definition of finitely describeable streams we give the definition of an uncertain LOLA semantics:

\begin{definition}[Uncertain Lola semantics]\todo{Maybe make semantics
denotional} Given a finitely describable input sream set $\Sigma$
described by $\sigma \in \mathcal{S}_{\mathbb{B}^\star}$ and a
specification $\varphi$ the uncertain semantics of an expression
$\llbracket \cdot \rrbracket_{\varphi}: E_\mathbb{D} \rightarrow
\mathbb{D}^\star$ is iteratively defined as:

\begin{enumerate}
 \item $\llbracket c \rrbracket_{\varphi}(t) = c$
 \item $\llbracket s[o,c] \rrbracket_{\varphi}(t) = \begin{cases}
s_i^{t+o} & \textrm{if } t + o \in \mathbb{T} \textrm{ and } s = s_i
\textrm{ (input stream)}\\ \llbracket e \rrbracket_{\varphi}(t + o) &
\textrm{if } t + o \in \mathbb{T} \textrm{ and } s \textrm{ is defined
via } s = e\\ c & \textrm{else}
                                    \end{cases}$
 \item $\llbracket f(e_1,...,e_n) \rrbracket_{\varphi}(t) =
\texttt{f}(\llbracket e_1 \rrbracket_{\varphi}(t), ..., \llbracket e_n
\rrbracket_{\varphi}(t))$
 \item $\llbracket ite(e_1, e_2, e_3) \rrbracket_{\varphi}(t) =
\texttt{ite}(\llbracket e_1 \rrbracket_{\varphi}(t), ..., \llbracket
e_n \rrbracket_{\varphi}(t))$
\end{enumerate}

The symbolic semantics of a specification $\varphi$ where every output stream $s'_i$ is defined by an expression $e'_i$ is consequently defined as:\\

\noindent
$\llbracket \varphi \rrbracket^\textrm{symb} = (\llbracket e'_1  \rrbracket_{\varphi}, ..., \llbracket e'_m \rrbracket_{\varphi})$\\

Together with the constraints from the input streams one receives the uncertain semantics as the set of all streams that model the symbolic semantics:\\

\noindent
$\llbracket \varphi \rrbracket^\textrm{unc}: \mathcal{S}_{\mathbb{B}^\star} \rightarrow 2^{\mathcal{S}_{\mathbb{D}'_1} \times \dots \mathcal{S}_{\mathbb{D}'_m}}$\\
$\llbracket \varphi \rrbracket^\textrm{unc}(\sigma) = \{(s_1,\dots,s_m) | \forall t \in \mathbb{T}: (\forall i \leq t: \llbracket e'_1  \rrbracket_{\varphi}(i) = s_1(i) \land ... \land \llbracket e'_m  \rrbracket_{\varphi}(i) = s_m(i)) \models \sigma(t) \}$\\

\end{definition}

Based on this definition a monitor can be constructed which works as follows:

\begin{enumerate}
 \item Given: Lola Specification $\varphi$, Stream of input descriptions $\omega$.
 \item Set $t=0$
 \item For every output stream $s'_i$ defined by $s'_i = e_i$ calculate symbolic formula $\llbracket e_i \rrbracket_{\varphi}(t)$
       \footnote{Note: For not efficiently monitorable specification (infinite $+n$ loops) formulas may become infinitely large. In this case a special strategy for partial evaluation is required.} and add ${s'}_i^t := \llbracket e_i \rrbracket_{\varphi}(t)$ to set of pending outputs $\mathcal{O}$.
 \item Evaluate all expressions from $\mathcal{O}$ that do not contain variables $v^i$ with $i > t$ under the constraints $\omega(t)$ and print the output.
 \item Repeat from step 3 for timestamp $t := t + 1$ until $t + 1 \not\in \mathbb{T}$.
 \item Evaluate and print the remaining elements in $\mathcal{O}$
\end{enumerate}

Provided a suitable SMT-solver and decideability for the given logic, such a monitor can be constructed for every LOLA specification $\varphi$.

Note that it is not necessary for the monitor to calculate all symbolic formulas from scratch at every timestamp. If the specification is flattened, i.e. has exclusively $-1,0,+1$ offsets, the formulas from the last timestamp can be memorized and reused. Storage of formulas from more than one timestamp in the past is not necessary then. Specifications with future references may be rewritten to specifications without future references \todo{More details in introduction} or calculation may be postponed to the next step.

Additionally it is advisable to include a simplification step in the monitoring process to simplify the involved formulas as far as possible. Also when evaluation of an output event yields a constant value, all occurences of the associated variable in other formulas should directly be replaced by the value.

Also note that printing the outputs may be tricky depending on the concrete setting. The most exact representation of an output event is given by printing the corresponding symbolic formula together with the input constraints. However oftentimes it is sufficient to print a set of possible values or a window of reals. While this is an over-approximation, note that this just affects the printed outputs, while the internal calculation of further values is still based on symbolic formulas.

%# Idea: Pruning

\subsection{Pruning strategies}

Alas, there is a major drawback of the approach from the previous section, which especially plays a role in the field of Runtime Verification:

The symbolic formulas which are used for calculation may become arbitrarily complex. On the one hand there is a growing number of constraints, describing the input streams, on the other hand the set of atomic propositions on which the constraints are built may increase.

Note that in the field of static analysis this usually does not play a big role, since the determination of (possibly approximated) program invariants is finished after a finite, usually not too large number of iterations.
In the setting of Runtime Verification the calculation of uncertain values is repeated as long as input events arrive to the monitor, which, in the worst-case, may be infinitely long.
When performing Runtime Verification online, a special requirement is that the calculation time of the monitor is shorter than the time between arriving input events. As a consequence, a growing set of constraints and likewise a growing calculation time, is not acceptable for Runtime Verification.

To handle this issue a strategy to rewrite the formulas to build on a constant number of atomic propositions and a constant number of constraints, while still describing the same output streams, is required.
We call such a strategy a \textit{perfect pruning strategy}.
However they only exist for some logics.
For logics where it is not possible to find such a perfect pruning strategy, it is possible to use \textit{over-approximating pruning strategies}, i.e. those which reduce the set of atomic propositions and the number of constraints but the set of resulting output streams is a superset of the original one. In this case the uncertain calculation is not perfect anymore, but still sound.\todo{Theorem?}

%# Algorithm: Pruning

\subsection{Application to LOLA fragments}

In the following we will present perfect and over-approximating pruning strategies for the presented LOLA fragments in \cref{sec:lola}.

A first, common issue to solve is the set of input constraints which may grow with every timestamp. We make use of the fact that every event of the input constraint stream is a superset of the previous one.\todo{Change orig. def.} 
So our assumption is that the monitor only gets passed the difference between two subsequent input constraints; It internally has to store the relevant constraints from the past.

Sadly there is no general strategy to approximate or to cut down the stored set of previous input constraints.
Imagine a boolean stream $s = \langle s_0, s_1, \dots \rangle$ and a specification which checks if the current event is equal to the first event of the stream.
Imagine further all events are unknown, but for several events there is the additional knowledge that $s_i = s_0$.
In case for the event at timestamp $t$ the corresponding novel constraint would be $s_t = s_j$ for any $1 \leq j < t$. In this case it would be necessary to be able to recover all previous constraints to check if $s_j = s_0$ is known or not.\\

To overcome this issue we restrict ourselfs to a class of uncertain streams, where the possible values at timestamp $t$ only depend on the values from timestamps $t-n$ to $t$:

\begin{definition}[$n$-lookback Streams]
 A set of tuples of concrete streams $\Sigma \in 2^{\mathcal{S}_{\mathbb{D}_1} \times \dots \times \mathcal{S}_{\mathbb{D}_n}}$ with identifiers $\mathcal{S}$ is called an uncertain $n$-lookback stream, if
 it is finitely describable by a stream $\sigma \in \mathcal{S}_{\mathbb{B}^\star}$ such that\\
 
 \noindent
 $\forall t \in \mathbb{T} \backslash \{0\}: \sigma(t) \backslash \sigma(t-1) $ is a set of boolean constraints over atomic propositions  $\{s^i | s \in \mathcal{S}, i \in \mathbb{T} \textrm{ with } t-n \leq i \leq t \}$.
\end{definition}

Note that monitoring $n$-lookback streams does not mean, constraints with symbols referring to events more than $n$ timestamps ago can be removed from the set of input constraints.
Consider for example the constraint set $\{s_1^0 \rightarrow s_1^1, s_1^1 \rightarrow s_1^2, \dots, s_1^{t-1} \rightarrow s_1^t\}$ which describes a $1$-lookback stream, but neglecting one constraint may lead to an over-approximation.

\subsubsection{$\textrm{LOLA}_\mathbb{B}$}

Let $\varphi \in \textrm{LOLA}_\mathbb{B}$ be a LOLA specification with input stream identifier $\mathcal{S}_i = \{s_1, \dots, s_n\}$ and output stream identifier $\mathcal{S}_o = \{s'_1, \dots, s'_m\}$ within the Propositional Logic fragment.

First we deal with the special case, where the input stream is a $0$-lookback stream, i.e. all unknown events from the stream may only be fully unknown or depend on other input events fromt the same timestamp.

For a certain timestamp $t$ the monitoring algorithm from the previous section would yield symbolic formulas of the following shape:\todo{I think it is not clear yet that we do this optimization each step and then calculate on with the rewritten formula. Maybe rewrite this section and make that clearer.}\todo{Well...future references? --> Make rewriting clearer} \\

\noindent
${s'}_1^t = \psi_1(s_1^0, \dots s_n^0, \dots, s_1^t, \dots, s_n^t)$\\
$\vdots$\\
${s'}_m^t = \psi_m(s_1^0, \dots s_n^0, \dots, s_1^t, \dots, s_n^t)$\\

Furthermore it will store a constraint set $\mathcal{C}_t = \sigma(t)$\todo{Should somewhere define which kind of formulas the constraint set may contain} with formulas over $s_i^j$ with $1 \leq i \leq n$, $0 \leq j \leq t$.

The set of equations for the ${s'}_i^t$ can be written as a multiplication with boolean matrices\cite{...}:\\

\noindent
$ s'^t = \left(
\begin{array}{c}
{s'}_1^t\\
\vdots\\
{s'}_m^t
\end{array}
\right)
 =
\left(
\begin{array}{ccc}
\psi_1^t(\fa,\dots,\fa) & \dots & \psi_1^t(\tr,\dots,\tr)\\
\vdots & \vdots & \vdots\\
\psi_m^t(\fa,\dots,\fa) & \dots & \psi_m^t(\tr,\dots,\tr)
\end{array}
\right)
*
\left(
\begin{array}{c}
\neg {s}_1^0 \land \dots \land \neg {s}_m^t\\
\vdots\\
{s}_m^0 \land \dots \land {s}_m^t
\end{array}
\right)$

Note that the matrix fully encodes the formulas $\psi_1^t, \dots, \psi_m^t$. 
The matrix is a $2^{n(t+1)} \times m$\todo{Or the other way round?} matrix.
Relevant for our calculation is exclusively the fact how many different values the vector $s'^t$ can take. 
The possible values are the columns of the matrix. 
There can be at most $2^m$ of these vectors.
As a result it is possible to find adjusted formulas ${\psi'}_1^t, \dots, {\psi'}_m^t$ over $m$ fresh variables $v_1,\dots,v_m$, by just building a new matrix by removing duplicate vectors until the length of the matrix is the lowest possible power of 2. The $\psi'$ formulas can then be directly created as DNFs of the entries where there row vectors bear a $\tr$.

Still we have not cared about the constraint set $\mathcal{C}_t = \{c_1, \dots, c_p\}$. 
Note that  we can always consider this set as a single formula $\gamma^t = c_1 \land \dots \land c_p$ and represent the constraints this way in our monitor.
Using this representation we can add a line $c = \gamma(s_1^0, \dots s_n^0, \dots, s_1^t, \dots, s_n^t)$ to our system of equation and consider it in our simplification to receive
a pruned, but equivalent version $\gamma'$ of our constraint set over fresh variables $v_1,\dots,v_{m+1}$. Note that potentially one additional fresh identifier is required since the result vector has an additional element.

Applying this strategy the monitor is able to reduce all symbolic formulas to $m+1$ variables at every calculation step. Note that $m$ is a constant, determined by the specification but not the timestamp which is currently calculated. Hence this strategy has a constant monitoring overhead per step. Furthermore this strategy yields a perfect uncertain calculation\todo{Theorem with proof in appendix?}.\\

\todo{Example?}

If we consider $k$-lookback streams with $k \geq 1$ we cannot directly apply the method from above since the variables $s_i^{t-j}$ for $0 < j \leq k$ may be referenced by new constraints in the next timestamp, hence they have to be preserved in the rewritten formulas.

We can address this issue in the following way:

Consider the matrix form above as concatenation of $2^{n*k}$ sub-matrices where each matrix describes the formulas $\psi^t_1, \dots, \psi^t_m, \gamma^t$ for a fixed setting of the variables $s_i^j, 1 \leq i \leq n, t-k < j \leq t$. These matrices can be simplified with the strategy explained above and concatenated again.
As a result one receives formulas over $s_i^j, 1 \leq i \leq n, t-k < j \leq t$ and $m+1$ fresh identifiers.

Since $n,k,m$ are constants the monitoring overhead for this strategy can still be considered constant. However if $n$ is not only a very small number the calculation time per step may be to high. However in practice uncertain streams usually have a quite low lookback. Another strategy to overcome this drawback is to wait for the calculation of timestamp $t$ until inputs up to timestamp $t+n$ have arrived. Then only those variables have to be preserved which are really used in the constraint set $\mathcal{C}_{t+n}$.

\subsubsection{$\textrm{LOLA}_\mathcal{LA}$}

Let $\varphi \in \textrm{LOLA}_\mathcal{LA}$ be a LOLA specification with input stream identifier $\mathcal{S}_i = \{s_1, \dots, s_n\}$ and output stream identifier $\mathcal{S}_o = \{s'_1, \dots, s'_m\}$ within the Linear Algebra fragment.

Principally we can apply the same trick for rewriting the symbolic formulas as for the Propositional Logic fragment.
The symbolic formulas we receive during monitoring step $t$ have the following form:\\

\noindent
${s'}_1^t = \sum\limits_{i=1}^{n} \sum\limits_{j=0}^{t} c_{1,i}^j \cdot s_i^j + o_1^t$\\
$\vdots$\\
${s'}_m^t = \sum\limits_{i=1}^{n} \sum\limits_{j=0}^{t} c_{m,i}^j \cdot s_i^j + o_m^t$\\

where the $c_{k,i}^j$ and $o_k^t$ are constant values.
This special form is guranteed since all stream are defined by Linear Algebra Expressions.

Furthermore let the input stream be a $k$-lookback stream, i.e. we do not want to prune variables $s_i^j$ for $j \in \{t-k, \dots, k\}$.
Again we can see this symbolic formulas as Matrix multiplication:

\scalebox{0.8}{
$s'^t = \left(
\begin{array}{c}
{s'}_1^t\\
\vdots\\
{s'}_m^t
\end{array}
\right)
 =
\left(
\begin{array}{ccc}
c_{1,1}^0 & \dots & \psi_{1,n}^{t-k-1}\\
\vdots & \vdots & \vdots\\
c_{m,1}^0 & \dots & \psi_{m,n}^{t-k-1}\\
\end{array}
\right)
*
\left(
\begin{array}{c}
s_1^0\\
\vdots\\
s_n^{t-k-1}
\end{array}
\right)
+
\left(
\begin{array}{ccc}
c_{1,1}^{t-k} & \dots & \psi_{1,n}^t\\
\vdots & \vdots & \vdots\\
c_{m,1}^{t-k} & \dots & \psi_{m,n}^t\\
\end{array}
\right)
*
\left(
\begin{array}{c}
s_1^{t-k}\\
\vdots\\
s_n^t
\end{array}
\right)
+
\left(
\begin{array}{c}
o_1^t\\
\vdots\\
o_m^t
\end{array}
\right)$
}

Note that the first matrix, say $M$, is an $(n(t-k)) \times m$ matrix. 
For the rank $r$ of the matrix we have $r \leq \min\{n(t-k),m\}$.

Hence we can find a $r \times n$ matrix $B$ (basis of $M$) such that: $\{y \in \mathbb{R}^{m} | \exists y \in \mathbb{R}^{n(t+1)}: y = Mx\} = \{y \in \mathbb{R}^{m} | \exists y \in \mathbb{R}^{r}: y = Bx\}$, i.e. the set of values which can be generated by $M$ is the same as the one that can be generated from $B$.
Additionally we can calculate a Basis-Change matrix $C$ s.t. $M*C = B$

From this matrix $B$ we can retrieve rewritten formulas with less coefficients and values:

\noindent
${s'}_1^t = \sum\limits_{i=1}^{r} c_{1,i} \cdot s_{1,i} + \sum\limits_{i=1}^{n} \sum\limits_{j=t-k}^{t} c_{1,i}^j \cdot s_i^j + o_1^t$\\
$\vdots$\\
${s'}_m^t = \sum\limits_{i=1}^{r} c_{m,i} \cdot s_{m,i} + \sum\limits_{i=1}^{n} \sum\limits_{j=t-k}^{t} c_{1,i}^j \cdot s_i^j + o_m^t$\\

In these formulas $s_{j,i}$ are fresh variables. With this strategy the monitor is able to cut down the symbolic formulas to a constant length of maximum $\mathcal{O}(m+k)$ at every timestamp and proceed calculation with the resulting formulas.

However we have not yet taken into account the constraint set $\mathcal{C}^t$ which may contain restrictions for the variables $s_{j,i}$ s.t. they cannot take any value in $\mathbb{R}$.

We handle this constraint set in the following way:

\begin{itemize}
 \item For all fresh variables $s_{i,j}$ calculate a minimum $\mu_{i,j} \in \mathbb{R}$ and maximum value $\nu_{i,j} \in \mathbb{R}$ such that all constraints in $\mathcal{C}^t$ are fulfilled with the additional constraints $v^t*M*C = s*B$, where $s$ is the vector of the fresh variables and $v$ the vector of $s_1^0,\dots,s_n^{t-k-1}$.
 \item Use the strategy from the previous section to reduce the variables in $\mathcal{C}^t$ to eliminate the variables $s_1^0,\dots,s_n^{t-k-1}$ from $\mathcal{C}$.\todo{Give abstract approach in previous section, give Details how to deal inequalities.}
 \item Add constraints from step 1 to the rewritten constraint set.
\end{itemize}

Note that by application of this algorithm we will not in all cases receive perfect results:

\begin{theorem}
 The presented approach yields a perfect uncertain calculation if all input constraints have the form $v = c$, where $v$ is an atomic proposition and $c$ a constant or atomic proposition.
\end{theorem}

\begin{theorem}
 There is no perfect uncertain calculation for $\textrm{LOLA}_\mathcal{LA}$ with constant memory.\todo{Actually our pruning algorithm is not with constant memory as well --> Define our notion of memory somewhere.}
\end{theorem}

\subsubsection{$\textrm{LOLA}_{\mathbb{B}/\mathcal{LA}}$}

Consider for example the following LOLA specifiaction

\begin{lstlisting}[mathescape]
 In i: Real
 In a: Real
 In b: Real
 
 Def x =     x[-1, 0] + i[0,0]
 Def y = 2 * y[-1, 0] + i[0,0]
 
 Def equality = (a == x) && (b == y)
\end{lstlisting}

Now imagine all the values of stream $x$ are unknown until timestamp $2$, but for each $i^j$ we have the constraint $0 \leq i^j \leq 1$.
The unpruned symbolic formulas describing the values of $a,b$ at timestamp $2$ would then be\\

\noindent
$
x^t =     i^0 +     i^1 + i^2\\
y^t = 4 * i^0 + 2 * i^1 + i^2\\
$

in Marix-Notation:\\

$\left(
\begin{array}{c}
x^t\\
y^t
\end{array}
\right)
 =
\left(
\begin{array}{ccccc}
1 & 1 & 1\\
4 & 2 & 1\\
\end{array}
\right)
*
\left(
\begin{array}{c}
i^0\\
i^1 \\
i^2
\end{array}
\right)$\\

Since the constraints for the input streams force all $i^j$ to be between $0$ and $1$ the possible set of value combinations $x$ and $y$ can take at timestamp $t$ is described by
a polyhedron with 8 edges depicted in \cref{fig:polygon}.

\def\nudge{.5}

\tikzset{axis/.style={ultra thick, black, -latex, shorten <=-\nudge cm, shorten >=-2*\nudge cm}}

\begin{figure}[h!]

\begin{tikzpicture}
%\draw[axis] (0,0) -- (8,0) node[right=2* \nudge cm] {\(a\)};
%\draw[axis] (0,0) -- (0,3) node[above=2*\nudge cm] {\(b\)};

\tkzInit[xmax=8,ymax=3,xmin=-.5,ymin=-.5]
%\tkzGrid
\tkzAxeXY[/tkzdrawX/label=$x^3$,/tkzdrawY/label=$y^3$]

\fill [blue!50] (0,0) -- (4,1) -- (6,2) -- (7,3) -- (3,2) -- (1,1) -- (0,0);

\draw [-stealth,line width=.7pt] (0,0) -- (4,1);
\draw [-stealth,line width=.7pt] (0,0) -- (2,1);
\draw [-stealth,line width=.7pt] (0,0) -- (1,1);
\end{tikzpicture}

\caption{Set of possible value combinations of $x^3$ and $y^3$}
\label{fig:polygon}
\end{figure}


However to describe a polygon with 6 edges.
Since we have no information on the values which arrive on streams we cannot approximate this set of possible values by another shape without loosing perfectnes.
But a polygon with 6 edges can only be described with 3 vectors, i.e. in a formula with four atomic propostions.

It is easy to see that with each new arriving, unknown input you get a new vector added to your matrix, which is not a linear combination of the others, hence for $n$ unknown inputs on stream $i$ the set of possible value combinations for $(x,y)$ is described by a polygon with $2n$ edges and for a perfect representation $n$ atomic propositions are required.

This example shows, that for the LOLA fragment $\textrm{LOLA}_{\mathbb{B}/\mathcal{LA}}$ there is no pruing strategy which leads to a perfect uncertain calculation.


\subsubsection{$\textrm{LOLA}_{\mathbb{B}/\mathcal{LA}}^+$}

In difference to the previous case the fragment $\textrm{LOLA}_{\mathbb{B}/\mathcal{LA}}^+$ also supports if-then-else expressions.

If you have a stream definition of form $s = ite(c,t,e)$ where $t$ and $e$ are of Boolean then it can be rewritten to $s = (c \land e) \lor (\neg c \land e)$, which is already part of $\textrm{LOLA}_{\mathbb{B}}$.
On the other hand, if you have $s = ite(c,t,e)$ where $t$ and $e$ are expressions of type Real the following can be done: 
The specification can be rewritten to handle $s$ as an input stream and at each monitoring step the constraint $s^t = (\llbracket c \rrbracket_\varphi \land \llbracket t \rrbracket_\varphi) \lor (\neg \llbracket c \rrbracket_\varphi \land \llbracket e \rrbracket_\varphi)$\todo{Adjust it according to the final def. of uncertain LOLA semantics.} can be added to the current set of constraints. After application of this strategy the specification is within the $\textrm{LOLA}_{\mathbb{B}/\mathcal{LA}}$ fragment and as a consequence the (sound but imperfect) pruning algorithms from there can be applied.

%# Proof Pruning: Perfectness

\subsection{Assumption-based Runtime Verification}

In the field of Runtime Verification an intensively studied topic are assumptions\cite{...}.
The basic idea is that assumptions, i.e. additional knowledge about the system which is observed, can be used to receive verdicts more precisely or earlier\cite{...}.
As a simple example imagine a monitor which is a property $p$ holds in every step ($\varphi = \mathcal{G}(p)$ in LTL). If one additionally has the assumption that if property $q$ holds in one state $p$ never holds in the next one ($\mathcal{G}(q \rightarrow X(\neg p))$), one would be able to construct a monitor which would be able to detect a violation of the correctness property $\varphi$ in the trace $\{p\}\{p,q\}\{\}...$ already at the second state.

Such assumptions play a very special role when dealing with uncertain inputs. 
Imagine monitoring a car during driving, where a speed sensor passes the current fuel consumption to a Runtime monitor every second to calculate the average fuel consumption during the last 10 minutes and raises an alarm if the average consumption was too high.
If the sensor is corrupted and sometimes fails to pass a valid value to the runtime monitor, the monitor would not be able to yield a valid verdict because the missing sensor value could be infinitely high and hence also the average could be infinitely high.
However, if we have the additional assumption that the current consumption rate may never be higher than 200\% of the last one, the monitor could in some cases still be able to detect that the average fuel consumption is ok.

The approach of symbolic Runtime Verification can perfectly be combined with assumptions about the system.

